Beyond $L_p$ clipping: Equalization-based Psychoacoustic Attacks against ASRs

Automatic Speech Recognition (ASR) systems convert speech into text and can be placed into two broad categories: traditional and fully end-to-end. Both types have been shown to be vulnerable to adversarial audio examples that sound benign to the human ear but force the ASR to produce malicious transcriptions. Of these attacks, only the "psychoacoustic" attacks can create examples with relatively imperceptible perturbations, as they leverage the knowledge of the human auditory system. Unfortunately, existing psychoacoustic attacks can only be applied against traditional models, and are obsolete against the newer, fully end-to-end ASRs. In this paper, we propose an equalization-based psychoacoustic attack that can exploit both traditional and fully end-to-end ASRs. We successfully demonstrate our attack against real-world ASRs that include DeepSpeech and Wav2Letter. Moreover, we employ a user study to verify that our method creates low audible distortion. Specifically, 80 of the 100 participants voted in favor of all our attack audio samples as less noisier than the existing state-of-the-art attack. Through this, we demonstrate both types of existing ASR pipelines can be exploited with minimum degradation to attack audio quality.

==> broad_impact.tex <==
\section{Broader Impact}\label{broader_impact}
This attack has demonstrated the additional fragility of ASR systems. While previous psychoacoustic attacks had become obsolete against fully end-to-end models, our attack demonstrates that such systems remain vulnerable inspite of this significant architectural change. The success of our attack (and others) against ASRs is primarily due to their improper modeling of human speech. This has resulted in lack of ASR robustness to such attacks. Future researchers can use our findings to ascertain the robustness of their ASRs using our attack. They can also study our attack and the vulnerability it exploits to build more robust models in the future.

Our work could both be used for potentially malicious and positive purposes. For example, an attacker might use our work to exploit ASRs (such as Siri and Alexa), forcing them to make unapproved bank transactions. On the other hand, a dissident can use the same attack to evade telephony surveillance systems. Authoritarian governments often use ASRs as part of their surveillance pipeline~\cite{abdullah2019kenensville}. They capture millions of hours of phone call audio then transcribe it using ASRs. Simple keyword  searches can be run on these transcripts to identify dissidents. A dissident, with knowledge of the ASR, can potentially use our attack to circumvent this surveillance infrastructure. The dissident can force the ASR to create chosen transcriptions such that the keyword search results turn up empty.


==> derivation.tex <==
\section{Adversarial Examples}

\subsection{Psychoacoustic Model}
Defines the criteria for ascertaining whether two audio samples are perceptibly indistinguishable from each other.
The two criteria the model uses are non-linear perception and frequency masking of audio frequencies.
\paragraph{Non-Linear Perception}
The first step of the psychoacoustic model involves taking the magnitude STFT of the signal, which is just an magnitude FFT over a moving window moving across the entire signal. Signal is broken into overlapping frames. The FFT operation is then applied to the frames. The output of the STFT is a matrix, with time on x-axis and frequency on y-axis.  Each bin of the matrix contains the intensity of frequency. This is because audio signal change quickly overtime the STFT can capture the nuances changes between the windows.

\begin{equation}
    %  X(m,\omega )=\sum _{n=-\infty }^{\infty }x[n]w[n-m]e^{-j\omega n}
    X(m,\omega ) = \mathbf {DFT}_w(x \cdot \mathbf {SHIFT}_{mR}(\omega))
    \label{stft}
\end{equation}
where $x$ is the input signal, $w$ is the windowing function, $m$ index of ....


\begin{equation}
p_X(m ,\omega ) = |X(m ,\omega )|^{2}
\label{magnitude_stft}
\end{equation}
 Next, the intensity of the frequency are scaled according the psychoacoustic perception of the human ear. All frequencies are not equally important to the human ear. Instead, it perceives frequencies non-linearly (i.e., gives more importance to certain frequencies over others). Specifically, the human ear places greater importance to the lower frequencies (0 to 1kHz) than to higher ones (15kHz to 20kHz). This is done using the bark scale.  
 
 Can be scaled using the Bark.
\begin{equation}
{\displaystyle {\mathbf{BARK}}=[(26.81f)/(1960+f)]-0.53\,}
\end{equation}
where f is the frequency. 




\subsection{Why vanilla PGD is poor for audio}
PGD has been been frequently used in the image space for controlling the adversarially introduced distortion.
It requires clipping the perturbation using some Lp norm.
However, in this subsection, we will argue that the vanilla PGD method is insufficient for audio distortions. 

The goal of the attacker is to produce imperceptible perturbations to an audio sample. The distortion is only imperceptible if it satisfies constraints described in the Psychoacoustic Model (Section()), namely auditory masking and non-linear frequency distortion:

\paragraph{Auditory Masking:}
Ask tom

\paragraph{Non-Linear frequency distortion:}
As discussed in Section Psychoacoustics, the human ear's perception of frequencies is non-linear. Lower frequencies are easier to hear than high frequencies, if the intensity for both are kept constant. Lp based clippings do not take these into account. Lets assume that an Lp based clipping results in a distortion, $\delta$, that we can add to the input audio $x$. This will result in an adversarial audio $x_{adv}$:
\begin{equation}
     x_{adv} = x + clip_{Lp}(\alpha\delta,\beta,-\beta)
     
\end{equation}
\begin{equation}
x_{adv} = x + N\delta    
\end{equation}
where $\alpha$ is the scaling factor.

We use the DFT to observe the effects of perturbation $\alpha\delta$ in the frequency domain. According to the \textit{put law here}, we employ the \textit{put law here}, multiplication in the time domain results in multiplication in the frequency domain. 

\begin{equation}
     DFT(N\delta) =  N DFT(\delta)
\end{equation}
where DFT is the Discrete Fourier Transform. As result, the frequencies will be added in the frequency domain:
\begin{comment}
%C: OLD EQUATION
\begin{equation}
     F[\alpha \delta_1] =  \alpha F(\delta_1), \
     ...\
     ,\
     \alpha F[ \delta_n] =  \alpha F(\delta_n), 
\end{equation}
\end{comment}

\begin{equation}
    F(N \delta) = \sum_{k=1}^{n} N_k F(\delta_k) = N F(\delta)
\end{equation}

where $n$ is the number of frequency points for a given signal $X$.

Looking at the above equation, we see that the epsilon is being adding equally across all frequencies of the audio sample. This creates an issue. Ideally, the epsilon should have a larger value for higher frequencies and lower value for lower frequencies. This will mean that we can larger degree of distortion in the higher frequencies without being perceived by the human ear. This linear addition of distortion equal across all frequencies violates the non-linear addition. 

What we want instead is a weighted scaling of the frequencies of the perturbation. Specifically, we want ${\alpha_1,...,\alpha_n}$, where each $\alpha$ is unique and has a value corresponding to the importance of the frequency to the human ear:
%C: OLD EQUATION
\begin{comment}
\begin{equation}
     F[\alpha_1 \epsilon_1] =  \alpha_1 F(\epsilon_1), \
     ...\
     ,\
     \alpha_n F[ \epsilon_n] =  \alpha_n F(\epsilon_n), 
\end{equation}
\end{comment} 
 
\begin{equation}
    F(\alpha_n \delta_n) = \sum_{k=1}^{n} \alpha_k F(\delta_k) = \alpha_n F(\delta_n)
\end{equation}


\begin{equation}
     clip(\alpha\delta,\beta)
\end{equation}






%delta = 1,2,4,2,5,11,1, -11
%alpha = 1
%beta = 10

%L_inf clip = 1,2,4,2,5,10,1, -10

==> methodology.tex <==
\section{Methodology} 
\subsection{Two Step Attack}
The attack consists of two steps. The first step generates the perturbation via gradient calculation. The next step uses psychoacoustics to project the gradients before adding them to the original audio file. METNION THAT THE ATTACK Iterative

\paragraph{Part 1: Perturbation Generation}
MOVE THIS INTO THE NEW SECTION 4. Now we can launch a two step attack to generate adversarial audio samples. There a number of ways to produce the $\delta$ (Equation~\ref{eq:simple_attack}). In our case, we employ the Fast Gradient Sign Method (FGSM)~\cite{} from the image:
\begin{equation}
    \delta = \epsilon\cdot\text{sign}(\nabla_xl(\theta, x, y))
\end{equation}
where $\epsilon$ is a variable to control the size of the perturbation, $\theta$ are the ASR parameters and $l$ is the loss. YOU ARE MOVING IN THE DIRECITON TO MINIMIZE THE LOSS. SPECIFY WHAT Y IS HERE. IT IS THE ATTACKER TRANSCRIPTION. Candidate perturbatnio. Just moves in the durection of the loss.

MAKE NEW 4.1. HERE YOU GIVE 
WE PROJECT THIS CANDIDATE PERTURBATION INTO A PSYC SOMETHING.
USE PSUDO CODE FOR THE ATTACK

\paragraph{Part 2: Projecting the Perturbation}

Using a single variable $\epsilon$ to scale the perturbation results in a linear scaling each frequency. As mentioned earlier, the human ear hears frequencies in a non-linearly. To overcome this issue, we replace the linear scale factor with the a psychoacoustic clipping:
% \begin{equation}
%     \delta = \epsilon*\text{sign}(\nabla_xl(\theta, x, y)) \\
% \end{equation}
\begin{equation}    
    \delta^* = \text{pclip}(\frac{\delta}{\epsilon})
\end{equation}
where pclip is a function that clips using the psychoacoustic model.  Specifically, we first generate the masking thresholds, using the psychoacoustic model, for the unaltered audio sample. The masking thresholds define the constraints for each frequency in the audio. To apply these constraints, the mSTFT has to be applied to $\delta$. However, clipping of the mSTFT $\delta$ is non-trivial as the mSTFT operation is non-invertible. At this point, the phase information is lost and overlapping nature of the mSTFT widows makes it difficult to recover the time domain represetation of the clipped signal.

Fortunately, the pclip function is designed to overcome these limitations.  


\subsection{ASR Model}
We test our attack against the DeepSpeech~\cite{} model. The model pipeline consists of an STFT stage followed by convolutions and bi-direcitonal RNNs. The model was trained on the LibriVox data set to achieve the state-of-the-art word error rate of 8\%~\cite{}.

Though this is not a pure end-to-end model (due to the existence of the STFT stage) we can treat it as such. This is done by applying the psychoacoustic projection on the raw audio instead of during propagation (as done in other attacks).  As a result, our attack can work against both end-to-end and non end-to-end models. In contrast, other psychoacoustic attacks~\cite{} can only execute against non end-to-end models.




